Simple totally disconnected locally compact groups separated by finiteness properties

We construct a sequence of simple non-discrete totally disconnected locally compact (tdlc) groups separated by finiteness properties; that is, for every positive integer $n$ there exists a simple non-discrete tdlc group that is of type $F_{n-1}$ but not of type $F_n$. This generalizes a result for discrete groups of Skipper--Witzel--Zaremsky. Furthermore, we construct a simple non-discrete tdlc group that is of type $FP_2$ over $\mathbb{Z}$ but not compactly presented. Our examples arise as Smith universal groups $\mathcal{U}(M, N)$ associated to permutation groups $M$ and $N$. We generalize a theorem of Haglund--Wise to tdlc groups and show that under mild conditions on $M$ and $N$ the finiteness properties of $\mathcal{U}(M, N)$ reflect those of its local actions $M$ and $N$.

==> packagefactor.tex <==
\makeatletter
\newlength{\factor@zaehlerhoehe}
\newlength{\factor@nennerhoehe}

 \DeclareRobustCommand*{\factor}[3][]
{%
{\mathpalette{\factor@impl@}{{#1}{#2}{#3}}}%
}
\newcommand*{\factor@impl@}[2]{\factor@impl#1#2}
\newcommand*{\factor@impl}[4]{
    \settoheight{\factor@zaehlerhoehe}{\ensuremath{#1#2{#3}}}%
    \settoheight{\factor@nennerhoehe}{\ensuremath{#1#2{#4}}}%
    \raisebox{0.3\factor@zaehlerhoehe}{\ensuremath{#1#2{#3}}}%
    \mkern-1mu /\mkern-1mu%
    \raisebox{-0.3\factor@nennerhoehe}{\ensuremath{#1#2{#4}}}%
}

 \DeclareRobustCommand*{\factortext}[3][]
{%
{\mathpalette{\factortext@impl@}{{#1}{#2}{#3}}}%
}
\newcommand*{\factortext@impl@}[2]{\factortext@impl#1#2}
\newcommand*{\factortext@impl}[4]{
    \settoheight{\factor@zaehlerhoehe}{\ensuremath{#1#2{#3}}}%
    \settoheight{\factor@nennerhoehe}{\ensuremath{#1#2{#4}}}%
    \raisebox{0.2\factor@zaehlerhoehe}{\ensuremath{#1#2{#3}}}%
    \mkern -2mu / \mkern-1mu%
    \raisebox{-0.2\factor@nennerhoehe}{\ensuremath{#1#2{#4}}}%
}

 \DeclareRobustCommand*{\schlichting}[3][]
{%
{\mathpalette{\schlichting@impl@}{{#1}{#2}{#3}}}%
}
\newcommand*{\schlichting@impl@}[2]{\schlichting@impl#1#2}
\newcommand*{\schlichting@impl}[4]{
    \settoheight{\factor@zaehlerhoehe}{\ensuremath{#1#2{#3}}}%
    \settoheight{\factor@nennerhoehe}{\ensuremath{#1#2{#4}}}%
    \raisebox{0.1\factor@zaehlerhoehe}{\ensuremath{#1#2{#3}}}%
    \mkern -2mu /\!/ \mkern-1mu%
    \raisebox{-0.1\factor@nennerhoehe}{\ensuremath{#1#2{#4}}}%
}

 \DeclareRobustCommand*{\factorl}[3][]
{%
{\mathpalette{\factorl@impl@}{{#1}{#2}{#3}}}%
}
\newcommand*{\factorl@impl@}[2]{\factorl@impl#1#2}
\newcommand*{\factorl@impl}[4]{
    \settoheight{\factor@zaehlerhoehe}{\ensuremath{#1#2{#3}}}%
    \settoheight{\factor@nennerhoehe}{\ensuremath{#1#2{#4}}}%
    \raisebox{-0.3\factor@nennerhoehe}{\ensuremath{#1#2{#4}}}%
    \mkern-2mu\diagdown\mkern-4mu%
    \raisebox{0.3\factor@zaehlerhoehe}{\ensuremath{#1#2{#3}}}%
}

 \DeclareRobustCommand*{\factorltext}[3][]
{%
{\mathpalette{\factorltext@impl@}{{#1}{#2}{#3}}}%
}
\newcommand*{\factorltext@impl@}[2]{\factorltext@impl#1#2}
\newcommand*{\factorltext@impl}[4]{
    \settoheight{\factor@zaehlerhoehe}{\ensuremath{#1#2{#3}}}%
    \settoheight{\factor@nennerhoehe}{\ensuremath{#1#2{#4}}}%
    \raisebox{-0.2\factor@nennerhoehe}{\ensuremath{#1#2{#4}}}%
    \mkern 1mu\backslash\mkern 0mu%
    \raisebox{0.2\factor@zaehlerhoehe}{\ensuremath{#1#2{#3}}}%
}

\makeatother
